The High-Acceptance Dielectron Spectrometer HADES

HADES is a versatile magnetic spectrometer aimed at studying dielectron production in pion, proton and heavy-ion induced collisions. Its main features include a ring imaging gas Cherenkov detector for electron-hadron discrimination, a tracking system consisting of a set of 6 superconducting coils producing a toroidal field and drift chambers and a multiplicity and electron trigger array for additional electron-hadron discrimination and event characterization. A two-stage trigger system enhances events containing electrons. The physics program is focused on the investigation of hadron properties in nuclei and in the hot and dense hadronic matter. The detector system is characterized by an 85% azimuthal coverage over a polar angle interval from 18 to 85 degree, a single electron efficiency of 50% and a vector meson mass resolution of 2.5%. Identification of pions, kaons and protons is achieved combining time-of-flight and energy loss measurements over a large momentum range. This paper describes the main features and the performance of the detector system.

==> DetectorOverview/DetectorOverview.tex <==
\section{Detector overview}

HADES
exploits state-of-the art detectors and data acquisition systems combined
with a powerful electron trigger.

\begin{figure}[htb]
 % \vspace*{-.8cm}
 % \epsfxsize=12cm
 %  \epsfysize=3cm
\center
\includegraphics[width=10cm,height=10cm]{DetectorOverview/hades_cros.eps}
% \vspace*{-1cm}
\caption[]{Schematic layout of the HADES detector.
HADES has a toroidal geometry with 6 sectors. A RICH detector with
gaseous radiator, a carbon fiber mirror and an UV photon detector
with solid CsI photocathode is used for electron identification. Two
sets of Mini-Drift Chambers (MDC) with 4 modules per sector are
placed in front and behind the magnetic field to measure particle
momenta. A time of flight wall (TOF/TOFINO) accompanied by a
Pre-Shower detector at forward angles is used for additional
electron identification and trigger purposes. For reaction time
measurement, a START detector is located in front of the target.}
\label{hades}
\end{figure}

HADES is a large acceptance toroidal
spectrometer with six-fold symmetric azimuthal coverage. The
spectrometer acceptance covers polar angles between
$\theta=18^\circ$ and $\theta=85^\circ$. the target is
placed near the center of the Ring Imaging Cherenkov detector. HADES features six
identical sectors defined by the coils of the superconducting magnet.
The cross section of the detector in the vertical plane containing the
beam axis is shown in fig.~\ref{hades}. The angular and momentum
acceptance has been optimized for the detection of dielectron decays
of hadrons produced in the SIS energy regime.

Momentum reconstruction  is carried out by measuring the deflection
angle of particle trajectories derived from the hit positions in
four modules of the Mini-Drift Chambers (MDC) placed before and
after the magnetic field region.

Electron identification is performed with the hadron-blind gas Ring
Imaging Cherenkov detector (RICH), operating in a field-free region
together with the Multiplicity and Trigger Array (META) consisting
of time-of-flight scintillator walls (TOF/TOFINO) and
electromagnetic shower detectors (Pre-Shower).

A powerful multi-level trigger system is able to select events
within predefined charged particle multiplicity (first-level
trigger), as well as electron candidates.

In the following, a detailed description of the main
spectrometer components are given namely: beam detectors 
(chapter \ref{Chapter_start}), magnet (chapter \ref{Chapter_magnet}), RICH
(chapter\ref{Chapter_RICH}), tracking system (chapter
\ref{Chapter_MDC}) and META (chapter\ref{Chapter_tof} and chapter
\ref{Chapter_shower}). The detector description is followed by a
discussion of the data acquisition and trigger system 
(chapter \ref{Chapter_daq}) and the  data analysis framework 
(chapter \ref{Chapter_simana}). Finally, the detector performance is
discussed (chapter \ref{Chapter_simana}).

